Dynamic Semantic Occupancy Mapping using 3D Scene Flow and Closed-Form Bayesian Inference

This paper reports on a dynamic semantic mapping framework that incorporates 3D scene flow measurements into a closed-form Bayesian inference model. Existence of dynamic objects in the environment can cause artifacts and traces in current mapping algorithms, leading to an inconsistent map posterior. We leverage state-of-the-art semantic segmentation and 3D flow estimation using deep learning to provide measurements for map inference. We develop a Bayesian model that propagates the scene with flow and infers a 3D continuous (i.e., can be queried at arbitrary resolution) semantic occupancy map outperforming its static counterpart. Extensive experiments using publicly available data sets show that the proposed framework improves over its predecessors and input measurements from deep neural networks consistently.

==> related_work.tex <==
\section{Related work: Dynamic Semantic Mapping}

\subsection{Filtering out Dynamic Objects during Map Building}
\subsubsection{Geometric \& Deep Learning Approaches on Features}

Cheng et. al. \cite{cheng2020robust} proposed a method wherein they generate a point cloud map of the environment based on the localization result and then combine it with CRF-RNN-based semantic segmentation to generate a map. Results were compared to ORB-SLAM \cite{orbslam} for TUM-RGB dataset and shown to show much higher improvement in more dynamic sequences.

Brasch et al. \cite{brasch2018semantic} worked on a combining semantic information with a probabilistic model that rejects dynamic objects as outliers. Furthermore, they made an argument for utilizing descriptive ORB features over using direct methods, due to their sensitivity to illumination changes. In the event that a map point cannot be initialized with ORB features, their system falls back on using a resolution pyramid to do so. Each map point maintains a depth estimate \emph{d}, an inlier ratio $\phi$, that associates it with the stability of the map point, and a {\textcolor{red}{matching accuracy parameter}}, which are then used to evaluate whether a map point is static or dynamic. These results are then combined with semantic probabilities predicted by a CNN (Convolutional Neural Network) output, to dictate the semantics of a map point. The authors present results in dynamic environments with virtual KITTI, Cityscapes and Synthia against ORB-SLAM* as a benchmark. {\textcolor{purple}{While the authors' approach for fusing the observations with the matching accuracy parameter lends some confidence in tracking a feature correctly, the lack of instance level segmentation could lead to points being erroneously tracked in the case of two objects of the same semantic class "crossing over". Also, instead of tracking multiple features separately inside an semantic segmentation instance, wouldn't it be less computationally intensive to treat them as one abstraction? Essentially, all the features of one "semantic segmentation" instance may have similar depth information because they belong to the same object.}}

DynaSLAM \cite{dynaslam} is another such method where the authors combine a priori information about \emph{potentially dynamic} semantic classes with keypoint tracking and matching. Moreover, to deal with patches around keypoints being classified as dynamic, the variance in the depth image is factored into the labelling. The authors evaluated their results on the TUM RGB-D and KITTI dataset as well, where they compared their method to DVO-SLAM, DSLAM and ORB-SLAM2. On TUM-RGBD, they outperform DVO-SLAM and DSLAM and perform similar to ORB-SLAM2. On the KITTI dataset, better results are obtained in sequences which {\textcolor{purple}{contain more structural objects. The authors could track features on the basis of direct methods as a fail-safe if they are not able to extract keypoints from objects lacking texture or at a far away distance (as done by Brasch et al. \cite{brasch2018semantic}). The advantage of the approach is the distinction provided to objects that are "movable," so as to filter them on the basis of depth information and inpainting the background occluded by dynamic objects by leveraging multiple views. However, an obvious disadvantange is that a priori dynamic classes are neither tracked nor mapped despite having potentially useful information that could aid in pose estimation (eg. a person being static)}.}

DS-SLAM \cite{yu2018ds} combines semantic segmentation (using SegNet \cite{badrinarayanan2017segnet}) with a moving consistency check to filter out dynamic objects. The moving consistency check involves a pipeline for tracking features with optical flow, computing the fundamental matrix with RANSAC inliers to match points in subsequent keyframes and finally, rejcting outliers on the basis of distance from matched point to epipolar line. The work is evaluated on the TUM-RGBD dataset and compared to ORB-SLAM2 for ATE and RMSE. There is significant improvement observed in datasets that are more dynamic in comparison to the static ones. More recently, Cui and Ma proposed SOF-SLAM\cite{cui2019sof}, wherein optical flow coupled with semantic segmentation, is used for detection and removal of dynamic features. Results were evaluated on the TUM RGB-D dataset and comparisons were made with the RGB-D ORB-SLAM2 system as well as a version of ORB-SLAM2 that only uses semantic information to filter dynamic objects. They also compare results to DynaSLAM \cite{dynaslam}, DS-SLAM \cite{yu2018ds} and Detect-SLAM \cite{detect} for the $w_{halfsphere}, w_{rpy}, w_{static}$ and $w_{xyz}$ sequences. {\textcolor{purple}{As other work in this section, DS-SLAM completely eliminates dynamic objects from their semantic map-building framework and neither work utilizes optical flow for task other than discarding points that are mobile with respect to the sensor.}}

Another recent work, by Ma et al.\cite{ma2019dsod} builds a framework that employs a depth prediction network and semantic segmentation over a DSO \cite{dso} base. The depth prediction network is motivated by the uncertainty surrounding the initialized candidate points from the current key frame. High uncertainty could lead to false projection pairs being generated and the network narrows down the depth search interval for this candidate point. Semantic segmentation with Mask-RCNN is post-processed with a scalar representing the semantic label and the image is converted to a grayscale image. %A motion consistency check is done by matching key points from reference frames to the target projection points in the current observed frame - RANSAC - fundamental matrix
The points in the image are finally classified as static or dynamic after a motion consistency check and discarded for pose estimation. Results are evaluated on the KITTI dataset and compared to DSO with significant improvements in the translational root mean square error.

Chen et al. \cite{chen2019suma++} proposed a method to leverage semantic information to filter out dynamic objects. The map representation is in the form of surfels and the LiDAR point cloud attained is processed by using a spherical projection in the form of a vertex map. Using the vertex map, a normal map is also generated. RangeNet++ \cite{milioto2019rangenet++} is used to classify each point with a label and the classification results are back-projected onto the 3D point cloud. To filter out points dynamically, the authors check the semantic consistency between the new observation (where labels are taken into consideration) and the world model. If the labels are not compatible, the surfels are assumed to be dynamic and a stability log-odds ratio is updated to mark it so. The "unstable" surfels are not added to the map. The algorithm is evaluated on KITTI Road Sequences and KITTI Odometry benchmark and compare relative errors averaged over trajectories with SuMa \cite{behley2018efficient} and \cite{zhang2014loam}. \textcolor{purple}{Despite not tracking objects and removing surfels in the globally consistent map that are inconsistent with new semantic observations, the approach does not eliminate potentially dynamic semantic classes, which is advantageous and unlike approaches delineated previously in this review. However, the removal of surfels from the map is \emph{completely dependent} on the assumption that the semantic segmentation is foolproof and the inconsistency between the new observation and global map must mean that this point is dynamic. In case this happens, static objects that otherwise provide useful features for aligning point cloud scans will be removed and deteriorate performance. }

\subsubsection{Object-Oriented Approaches}
SLAM++ \cite{salas2013slam++} is another such method where each node in the map is in the form of homogeneous transformation of the object pose or historical pose of a handheld RGB-D camera. The authors use camera-model ICP to determine the pose and use individual object-camera relative pose estimates to cull out "moved" or "moving" objects from the pose graph later. Their work is demonstrated qualitatively. {\textcolor{purple}{The main disadvantage of this method is that the full set of object instances with their geometric shapes have to be known and initialized beforehand.}}

\subsubsection{Scene Flow Approaches}
Alcantarilla et. al. \cite{alcantarilla2012combining} discuss taking advantage of dense scene flow to increase the accuracy of SLAM in the presence of dynamic objects, using a stereo camera rig. Their approach involves computing dense scene flow from the right and left disparity map, 2D optical flow and 3D scene flow \cite{vedula1999three}. First, the motion vector for each of the pixels between frames is calculated. Second, the uncertainty (covariance matrix $\Sigma$) surrounding the scene flow vector is taken into account with the Jacobian of the scene flow with respect to the measurements and the measurement noise matrix. The residual motion likelihood is then computed with the motion vector M and the scene flow uncertainty $\Sigma$. This motion likelihood is applied in their visual odometry pipeline to filter out RANSAC inliers that could belong to dynamic objects. Their method is evaluated in scenes of railway stations and on crowded city streets. Adding on to the work by Alcantarilla et. al.\cite{alcantarilla2012combining}, in DOS-SLAM \cite{xu2019slam}, dynamic instance-based object segmentation is used for static semantic octo-map tree building. After performing instance-segmentation on RGB images with YOLACT, the authors use multi-view geometry to judge ORB-feature points that do not satisfy geometric constraints, as dynamic. This classification is based on epipolar geometry and the flow vector bound introduced in \cite{alcantarilla2012combining}. If the number of dynamic feature points on an object exceed a certain threshold, it is categorized as dynamic. The results are filtered in building a semantic octo-tree map. Results are evaluated on the TUM RGB-D dataset and compared to ORB-SLAM2 \cite{orbslam2}.

\textcolor{purple}{A global critique of work in this section - dynamic objects are not tracked or added to the map and simply ignored for the purpose of pose estimation. A SLAM framework where each scene has an object-level representation tracked with rigid scene flow. As SUMA \cite{behley2018efficient} is a base framework wherein a globally consistent map is made with the computation of rigid transformations between frames/scenes. Using rigid scene flow to estimate the velocity and transformation of each new object measurement with respect to a previous frame and then retroactively inserting it into a scene may prove helpful.}

\subsection{Leveraging or Propagating Dynamic Object Information} 

\subsubsection{Geometric \& Deep Learning Approaches on Features}

Zhong et. al. \cite{detect} proposed Detect-SLAM wherein each feature point is assigned a moving probability and propagated frame-by-frame while simultaneously being updated in the local map. Features extracted on moving objects are then removed before camera pose estimation. An object ID is predicted for every detected region in image space and an object point cloud is generated and transformed into the camera pose to be inserted into the object map. Another interesting aspect of the work is that the same object point cloud inserted into the map is projected into the 2D image plane to propose candidate regions with the same object. \textcolor{purple}{This particular step prevents frame-to-frame object initialization and tracking. Existing point cloud object is aiding in generating proposals in the detection thread, which are then assigned the same object ID.}  The algorithm was evaluated on TUM RGB-D dataset and the results were compared to \cite{orbslam}. {\color{purple} Although dynamic objects are tracked with the association of a moving probability, they are discarded for the purpose of pose estimation. }

Schorghuber et. al. \cite{schorghuber2019slamantic} propose a dynamics factor that combines information about \emph{how dynamic} a semantic class is with its detection consistency. This factor is then used to categorize 2D (image) feature-to-3D point matches as static, dynamic or static-dynamic. Static points are used to initialize a camera pose estimate, which is then used for geometric validation of the static-dynamic points. Valid 2D point matches in the "static" group and 3D point matches in the "static-dynamic" group are finally used to compute the final pose estimate. The method is motivated by being able to utilize classes that are \emph{expected to be dynamic} but are actually static in improving localization (e.g. a parked car). If the parked car, which was inculcated into localization, starts moving through the course of the SLAM process, it does not cause issues because it becomes "dynamic" in the dynamics factor classification. Moreover, not rejecting the semantic class of "car," for localization increases the number of points that can be used for pose estimation. Their method is evaluated on the Virtual-KITTI dataset where they outperform a ORB-SLAM2 \cite{orbslam2} baseline. Their results on Cityscapes demonstrated success in situations where the baseline fails. Additionally, results are compared to DynaSLAM \cite{dynaslam} on the KITTI and TUM datasets. {\color{purple} {While the work utilizes effectively features that would otherwise be considered dynamic, an obvious downside is that due to their dynamic nature, one needs more data for pose estimation when there are less features and only \emph{potentially dynamic} classes. Moreover, the "dynamics factor" is highly subjective to knowledge of semantic classes and parameter tuning.}}

Recurrent OctoMap is another semantic mapping approach that operates on 3D-LiDAR scans. Initially employing PointNet \cite{qi2017pointnet} (pre-trained on the KITTI dataset) to extract semantic features, the approach then moves to long-term localization on mapping. To do this a recurrent-OctoMap inherits functions from OctoMap \cite{octomap}, where the semantic observations and states are stores and with which, dynamic changes can be observed. New LiDAR scans and LiDAR odometry obtained from LOAM \cite{zhang2014loam} is used to transform the point cloud to a map frame. Each recurrent-OctoMap cell is assigned a semantic feature created by average pooling of these points. Dynamic objects are only kept in the map for five minutes in their experiments. Lastly, the authors propose to model the fusion of semantic observations with an LSTM \cite{lstm}. Results are validated on the ETH Parking Lot dataset with 4 categories of objects, and compared to a Bayesian update baseline.

\subsubsection{Object-Oriented Approaches}
Fusion++ \cite{mccormac2018fusion++} is another method where Mask-RCNN-generated instance segmentation is used to initialize reconstructions of objects after which, \textcolor{red}{they are fused with voxel foreground masks. Each voxel without an object has an existence probability association with it.}  Although the work does not focus on working with dynamic objects, local object tracking is done after initialization. The method is demonstrated on the TUM RGB-D dataset.

MaskFusion \cite{maskfusion} is another method where the SLAM system maintains a 3D representation of objects in a scene, which are tracked and fused over time by using object labels to associate surfels with the right model. Segmentation is done on an instance-level with Mask R-CNN \cite{maskrcnn} and the extracted masks are matched with geometric segmentation labels from an edginess-based depth map. Upon mask-label matching, a new object is initialized. \textcolor{red} {The pose of the model is tracked by jointly minimizing a geometric and photometric error function and the remaining surfel variables are updated by projective data association.} Results on ATE and RPE are compared to (more importantly) to VO-SF and Co-Fusion on slightly dynamic and highly dynamic sequences in the TUM RGB-D dataset. Their work performs better in highly dynamic scenarios. {\textcolor{purple}{The work depends on the known object models of its 80 semantics classes to do data association and is only limited to tracking rigid objects.}}


Huang et. al. developed ClusterSLAM \cite{huang2019clusterslam}, where rigid bodies are identified along with their rigid motion estimate. For a long-term assignment of a landmark, the authors first, describe the motion inconsistencies of multiple landmarks with a motion distance matrix and then, perform a hierarchical clustering approach to merge into the final static or dynamic rigid body. The shape and trajectory of landmarks are updated by a noise-aware point cloud registration and subsequent factor-graph optimization. Lastly, the approach chunks frames for pose graph optimization for the sake of efficiency;  however the quality of clustering increases with large chunk sizes but the accuracy decreases. The authors demonstrate their algorithm on KITTI and two synthetic datasets - SUNCG and CARLA and evaluate the ATE and RPE with, most importantly, tracking-by-semantic-segmentation. They also compare their real-time SLAM performance with DynSLAM \cite{barsan2018robust}. {\textcolor{purple}{ The authors provide a framework comparable to leveraging a semantic segmentation framework and eliminate semantic-geometric-object data association from the tracking pipeline, which may be advantageous. However, their method seems to rely on the quality of landmark extraction and data association and there being sufficient landmarks to detect an object. }}

Xu et. al \cite{xu2019mid} introduced MID-fusion - where the transform of the camera with respect to the world coordinates $T_{C_{L}W}$is tracked with geometric and photometric error using ICP. From each live frame, objects are retrieved after ray-casting from camera's estimated pose and then, using a modified error formulation for $T_{C{L}W}$, dynamic objects are marked (at an inlier ratio less than 0.9). Data association \textcolor{purple}{(Why this can't be real-time)} of objects in the map with the objects in the live frame is done by rendering the masks of existing objects and comparing them to Mask-RCNN\cite{maskrcnn}-generated masks via IoU. Dynamic objects are tracked every live frame with respect to the camera pose by estimating the associated transform ($T_{C_LO_L}$), but alignment is done for the vertex map in the live frame with that of the vertex map in a reference frame. The segmentation masks are further pruned after ICP is done again using photometric error by now aligning the reference map with the live frame instead. Using Vespa et. al.'s approach \cite{vespa2018efficient}, they leverage colour and geometric information to generate a TSDF and store this information into an associated voxel (semantics are averaged out instead of bayesian updates). New objects are initialized with their own coordinate frame with respect to the world frame and SDF by projecting pixels to world coordinates. Lastly, to spend less time on ray-casting, a foreground probability mask previously ascertained with Mask-RCNN is utilized. The authors compare their results with most notably DynaSLAM \cite{dynaslam} and MaskFusion \cite{maskfusion} on the TUM-RGB-D dataset. While they \textcolor{red}{outperform work focusing on dense approaches, they do not outperform DynaSLAM (feature-based)}. \textcolor{red}{Because the authors' have a separate coordinate system for each object, the reconstructions do not collide with each other. The authors' claim the quality of their reconstructions are superior to those as in MaskFusion, which relies on a surfel-based approach. Using octrees lends memory-efficiency, as discussed later in this literature review.} \textcolor{purple}{Some notable advantages of their approach are pruning the mask by incorporating motion of the object and using object-centric coordinate system instead of virtual camera tracking. The \textbf{quality of their reconstructions} were better than their counterparts and comparable to segmentation masks being initialized with ground-truth. However, the premise of their object tracking algorithm was to mask out human beings and to not track them. Moreover, their results are limited to indoor/table-top environments.}


\subsubsection{Scene Flow Approaches}
DynSLAM \cite{barsan2018robust} uses scene flow both for pose estimation and to track objects and make accurate reconstructions. The authors use a stereo setup to obtain instance segmentations, compute VO from scene flow and the depth map using ELAS or DispNet. Results of these three are then combined and separated into virtual frames - for background and each of the potentially dynamic objects. Using visual odometry, each new detection's motion is classified as static, dynamic or uncertain and then, initialized as a "virtual frame" containing only that object's data. The volumetric reconstruction of each object is then done with InfiniTAM using this "virtual frame" and the object's estimated 3D motion. The artifacts arising during reconstruction in outdoor environments causes the authors to use a garbage collection method to remove every voxel block that has a minimum TSDF value above a certain threshold. The authors evaluate the accuracy and completeness of their reconstruction method on the KITTI odometry and tracking datasets and demonstrate results with using ELAS and DispNet (DispNet performs far better on reconstruction completeness while ELAS on accuracy). {\textcolor{purple}{The obvious advantages of this approach are how the authors leveraged scene flow both for odometry and for classifying object motion. However, objects are tracked frame-by-frame on the basis of IoU (ie. some sort of data association) only and this can lead to erroneous tracking and fusing of results (even with information about depth map). This approach is also not robust to deformable objects like pedestrians, despite depth/scene flow information in their pipeline. Moreover, the garbage collection procedure done removes voxels after a certain step size has elapsed - their representation could be unsuitable for mapping applications? According to \cite{huang2019clusterslam}, DynSLAM also suffers from cumulative drift.}}

Ushani et. al. \cite{aushani-2018a} propose training a neural network pipeline for learning features from occupancy grid maps to aid in scene flow computation for LiDAR scans. The loss function is designed to increase distance between non-matched features and assign correct semantic class labels to all features. In the evaluation phase, an energy function serves as a metric for scene flow computation from a position $x_1$ in an occupancy grid map $G_t$ to another position $x_2$ in the map $G_{t+1}$ at the next time step (t+1). Therefore, it takes into account the learned distance between the features and the residual error for scene flow computation. Scene flow is computed by minimizing this energy function via the EM-algorithm. The E-step finds the latent variable $x_2$ in the map $G_2$ for every $x_1$ and the M-step updates the estimate of $x_1$ that led to scene flow to $x_2$. The authors evaluated their results on the KITTI dataset and compared their method to their previous approach of using occupancy constancy. Results on scene flow estimates of dynamic semantic classes were within an error margin of 30cm more than 88\% of the time.

Dewan et. al. \cite{dewan2016rigid} assume local geometric constancy to estimate a dense rigid motion field that explains the motion between two LiDAR scans. This is formulated as an energy minimization problem where the energy potentials fora data term (based on SHOT descriptors) and regularization term (based on creating a neighbourhood from LiDAR scans) are taken into consideration. The authors evaluate their method on the KITTI dataset for rigid-objects and four kinds of human body-arm motions for non-rigid objects and compare it to ICP and RANSAC-preprocessed ICP. Quantitative results are significant in the case of non-rigid objects. They also observe motion estimates of points farther away from the sensor to be different from those closer due to the higher rotational motion of the former; however, the estimates found are still accurate. 

\reorg
%Kochanov et. al. \cite{kochanov2016scene} in their paper use a probabilistic filtering technique that leverages scene flow to update occupancy and semantic belief. Each measurement is comprised by a depth map and a semantic segmenetation (p for each pixel). Additionally, they employ a CRF on top of the accumulated voxel grid to explain accumulated measurements in each frame (what does this mean??). Finally, they employ a clustering algorithm to group voxels together into object proposals using density-based spatial clustering. 

%they propose tracking of discovered objects and predicting occupancy according to motion??

FlowNet3d:

FlowNet3d can process two 3D point clouds scanned from two successive time steps and produce the scene flow for each point in the first point cloud. It consists of three layers that perform functions specific to capturing spatio-temporal relationships. The first layer, i.e., the point feature learning layer (also called the set conv layer) relies on farthest point sampling to obtain a smaller subset of region centres. These centres are used to learn a filter that extracts new local features in the region surrounding these centroids. The second type of layer, i.e., the flow embedding layer, takes both the point clouds P and Q into consideration and learns a filter similar to the set conv filter in the previous layers. The objective of this filter, however, is to compute for a point in the first point cloud the flow votes of the neighbouring points in the second point cloud. The flow embeddings are extracted using the Euclidean and feature distance between the points in the clouds. As the object of the DNN architecture is to estimate the flow of each point in the inputted point cloud, target points (computed from the flow embedding in the previous layer), together with the original point cloud are fed into an up convolution layer. The method upsamples point features according to its nearby points’ features rather than interpolate. Huber loss and a cycle-consistency loss based on shifting the second cloud back to the first one are utilised in the loss function. The authors also re-sample the input point clouds during inference and average the predicted flow. Their method is evaluated on the FlyingThings3D dataset and the KITTI scene flow dataset and results compared to PRSM, LDOF and OSF (which all used RGB-D or stereo) as input. The authors do not discuss any differences between using dense or sparse point clouds but outperform Dewan et al.’s work on rigid scene flow estimation. The main drawback of this work is that the complexity is linear with the number of points in the input point cloud. The convolution operations suggest high dependence on searching the neighbourhood of every point encountered within a specific radius.


HPLFlowNet

The idea behind HPLFlowNet is to take an input unstructured point cloud and enforce structure by storing it into a d-dimensional lattice, instead of grappling with performing a computation on each point individually. As the vertices of the Delaunay cell that contains a lattice point grows exponentially with dimensions, the authors compute a permutohedral grid by barycentric interpolation. Operation on the lattice is achieved by using a three-step convolution BCL (Bilateral Convolutional Layer) – the steps are \emph{splat – convolve – slice }, which is akin to gathering points into a d-dimensional lattice, performing sparse convolutions on them and then, interpolating the processed signals back to the same unstructured point cloud. This process replaces the vertices with d-simplices so that BCL has a performance comparable to one on a low-dimensional integer lattice. As the time and space complexity in BCL is linear in the number of points, the authors split BCL into two steps – a down-convolution (DownBCL) and up-convolution (UpBCL). A series of DownBCLs creates a sparse, volumetric representation of the unstructured point cloud, which becomes coarser at every layer in a manner that is independent of the input size. Similar to this, a UpBCL will act on making the spatial representation finer until slicing is done on the last layer. Using multiple convolutional layers in this way instead of a single BCL layer allows a "deeper" architecture and to reduce discrepancies arising from the asymmetry of barycentric interpolation.

This pre-processing step is exploited to “splat” together with two points clouds observed at consecutive time steps into the same permutohedral lattice. To compare the two point clouds and calculate the scene flow, the authors introduce CorrBCL – that takes into account the “patch” correlation between the neighbourhoods of two point clouds and leverage the maximum distance movable between scans to create these neighbourhoods in the first place. As the point cloud is sparse and of variable density, density normalisation is done when the input point cloud is “splatted” for the first time, and they later report it to help the network generalise better under variable point densities. The network architecture is such that the two consecutive point clouds are individually down-sampled with DownBCL, mixed together with subsequent CorrBCL layers and then sliced with the UpBCL layer. As the output at each layer is of a lattice at a larger or lower scale than the preceding layer, skip connections are added between the DownBCL and the UpBCL at the same scales. To ensure translational invariance, the relative pose between a point and its enclosing simplex is concatenated with the input signal at each layer. Lastly, the loss function used is the End Point Error loss. The authors compare their results to FlowNet3d, ICP, SPLATFlowNet and the original BCL on the FlyingThings3D dataset and the KITTI scene flow dataset and outperform their counterparts, arguing that it may be due to their approach towards enforcing a structured representation and pipeline for processing both the unstructured point clouds.

MotionNet:

In this work, similar to HPLFlowNet, the input point cloud is pre-processed into a pre-defined structure before being fed into the neural network architecture. For a given frame, all the past frames are transformed to the current coordinate system not only to take into account past frames as input but also, to aggregate more points to disambiguate static background from moving objects. BEV-map representation involves the creation of 2D pseudo-image from a 3D voxel lattice. Each cell is associated with a binary vector along the vertical axis, over which a 2D convolution can be applied. Each frame is stored as a BEV map, and a sequence of these 2D pseudo-images are fed into a spatio-temporal pyramid network. The STPN is composed of STC (spatio-temporal convolution) blocks, which is a sequence of two 2D convolutions and a degenerate 3D convolution, that works on the temporal domain. In order to learn at multiple resolutions, both the spatial and temporal convolutions are applied at multiple scales and then fused using global temporal pooling. The result is fed into the up-sampled layers for the decoder output. The objective of this work, contrary to the previous two, is to firstly, classify each BEV map cell category, secondly posit whether it is dynamic or not and thirdly to estimate where the cell will be moving to in the future. To effectively deal with jitter introduced in flow estimation by regressing future positions of cells (via L1 loss), the authors threshold the motion of cells that are considered background or static. The authors claim that their method can perceive “unobserved” objects better than by tracking a bounding box prediction. For the task of classification and state-estimation, the authors calculate a cross-entropy loss, weighted differently to mitigate class imbalance. Lastly, another composition of loss functions to capture spatio-temporal dependencies is used. It consists of a  spatial consistency loss, foreground temporal consistency loss (both of which are dependent on maximum motion possible between scans) and background temporal consistency loss (that acts on the transformation between background across frames). The authors evaluate their method on the nuScenes dataset and use five previous frames to each frame flow is computed for. The motion prediction performance is compared across 3 groups – static, slow ( < 5 m/s) and fast ( > 5 m/s) and average L2 displacement across scans are compared to the ground truth displacements. For classification, they report a cell classification accuracy. Results are benchmarked against HPLFlowNet, FlowNet3d and a static model of the environment, although models of the first two are trained on the FlyingThings3d dataset and not nuScenes.


\subsection{Map Representation}

Surfels v/s TSDFs : surfel surface unlike a TSDF can be moved without needing to update the truncation region around it. Surfels are similar to point clouds except they encode local surface properties like the radius and normal map. TSDF fusion methods apparently present some overhead due to having to switch representations between tracking and mapping. \cite{maskfusion}
\subsubsection{Truncated Signed Distance Functions}
Nie{\ss}ner et. al. \cite{neissner2013} argue that traversing hierarchical data structures like octrees leads to thread divergence in GPUs and the main failings of KinectFusion \cite{newcombe2011kinectfusion} are the computational burden and memory consumption. As an improvement, they introduce a new approach wherein voxels are projected onto incoming depth maps to construct corresponding TSDFs. Each voxel is swept to update the colour, SDF and weight and voxels outside the \textcolor{red}{truncation region of the observed surface} are marked as free-space. The TSDFs can be accessed, updated and deleted using a voxel hashing scheme that associates buckets with a 3D point in space. Within the bucket, there are hash table entries that point to a \textcolor{red}{voxel block that contains $8^3$ blocks}. In case the bucket is full, an offset variable is used to point to an entry corresponding to the same 3D point. Before the next depth image is stored, raycasting is done from the current camera pose to estimate the iso-surface. Using the depth and colour information from this iso-surface, point-to-plane projective ICP is done with the new depth map to estimate the new 6DOF camera pose. What is notable about this approach is \textcolor{red}{frame-to-model tracking is an improvement over frame-to-frame tracking that was reported in Newcombe et. al. \cite{newcombe2011kinectfusion} as suffering from drift.} \textcolor{red}{Another notable technique in the paper is the how surfaces are updated in the voxel. If the same surface is observed again in the current frustum, it is updated by means of a \textcolor{red}{running average}. Otherwise, it is primed for garbage collection. Garbage collection can be invoked when for a \textcolor{red}{voxel block}, the minimum absolute TSDF value exceeds a threshold or if maximum weight (that denotes "nearness" to sensor) is 0}. The authors compare their frame rates to extended (or moving volume) regular grids and the work by Chen et. al. \cite{chen2013scalable} that is based on a hierarchical approach. They also report the optimal bucket size (2), memory consumption (1G for voxels and 0.3G for hash tables) and resolution (8 mm) that gave them the best performance.

K\"{a}hler et al. \cite{KahlerPVM16} improve over areas otherwise unaddressed in Nie{\ss}ner et. al.'s work by aiming to \textcolor{red}{reduce memory consumption} and \textcolor{red}{increase speed}. Map-building is approached with the purpose of being multi-resolution i.e., to save memory on areas where fine resolution is not required and to provide higher resolutions on reconstructions that require finer detail. To incorporate this hierarchical structure to voxel hashing, the authors suggested hash tables be built at L levels and that the higher the level, the coarser the resolution of the data a hash entry is pointing directly to. If the hash entry is not directly pointing to a voxel and instead is pointing to a lower level, the resolution of the data stored will be finer. Block allocation is done similar to Nei{\ss}ner et. al.'s\cite{neissner2013} approach but contingent on which block the existing hash table is on. The decision of whether a finer resolution is required for a block is based on whether a node exceeds a complexity criteria that is dependent on roughness of the surface. Similary, the decision on whether a level should be at a coarser representation is made according to whether the children of a particular voxel block all fall below a particular complexity criteria. Upon splitting, eight blocks for children are allocated and the hash table entries are updated with an atomic compare-and-swap operation. Merging is done with subsampling and splitting with bilinear interpolation. To reconstruct the iso-surface via ray-casting, the pose of the camera needs to be known and specific care is taken when reading in interpolated values, especially when 2 out of 8 of the surrounding voxel blocks have a different resolution from the block being compared. The reconstruction results show improvement over an 8mm resolution uniform grid and closeness to a 2mm one. Moreover, 40-50\% of memory savings are reported. The interpolation scheme affects the frame-rate in comparison to K\"{a}hler et. al. \cite{kahler2015very} but is still 80-100 Hz. 

Amongst other improvements, InfiniTAM v3 \cite{prisacariu2017infinitam} builds upon Nie{\ss}ner et. al.'s work as the map representation but also \textcolor{red}{provides support for a surfel-based representation \cite{keller2013real}}, and a globally-consistent TSDF-based reconstruction that divides the scene into rigid submaps and optimizes the relative poses between them \cite{kahler2016real}.

Vespa et. al. \cite{vespa2018efficient} proposed an alternative oct-tree based map that can be rendered as a TSDF or occupancy map. To begin with, a representation is introduced wherein voxels are arranged sparsely \& non-contiguously and indexed with oct-trees. Voxel hashing is done with Morton codes, in order to be combine the ray-casting step of building a TSDF with tree-traversal. The tree-traversal order for all possible configurations is pre-computed and during a nearest-neighbour search or tri-linear interpolation the optimal configurations is chosen to select the optimal sampling point. Finally, the pipeline involves \begin{enumerate}\item tracking phase for frame-to-model alignment, where ray-casting is done over a point cloud generated from the depth, vertex and normal map and, \item a fusion phase to integrate this data into the map. \end{enumerate} In the fusion phase, a ray is marched along the line-of-sight within a particular bandwidth of the depth measurement, with which new parts of the scene are allocated into voxels introduced previously. (Note that the ray-marching is done from the root to the first intersected leaf node as in \cite{laine2010efficient}, performing tri-linear interpolation only near zero-crossings. Surface gradients are calculated via central difference on intersections.) Then, each voxel is projected into the current depth image with its known pose to compute the TSDF value. Finally, this TSDF is integrated into the global one using block averaging. \textcolor{purple}{ An interesting idea put forth by the authors is that both occupancy-grids and TSDFs are zero-crossings.}
The authors report the accuracy of their SLAM system with the RGB-D dataset and ICL-NUIM dataset, achieving lower ATEs than InfiniTAM \cite{prisacariu2017infinitam}. They also report total runtime on their fusion, raycasting and remaining steps.

Strecke et. al. \cite{strecke2019fusion} introduced EM-Fusion, which is an approach that deals with data association and occlusion handling with a probabilistic approach. The map and pose graph are updated by formulation as a MLE problem, wherein the posterior of the pose and map are maximized given depth images. Each pixel is associated to an object or alternatively, the background with a latent variable. The posterior is optimized separately for the camera pose and then, for the map. The map is stored by constructing SDFs that are stored in voxels and set up such that SDF value at a point within the grid is found through trilinear interpolation. The probability for each point in 3D space in any voxel belonging to the foreground/background is updated with the Mask-RCNN \cite{maskrcnn} segmentation likelihood. To account for occlusions, the authors only update regions where the Mask-RCNN-generated segmentation mask matches the projected mask of the object volume (determined via IoU by reprojecting object volume into image with raycasting). New objects are dealt with by associating an existence probability to new objects as in Fusion++ \cite{mccormac2018fusion++}. The posterior over the latent variable is approximated through the likelihood function. This likelihood is modelled with a mixture distribution according to whether the pixel falls inside the map volume of an object. Lastly, the authors track objects by following the approach in Bylow et. al. \cite{bylow2013real}, wherein only one trilinear interpolation lookup is done for data association of an incoming depth map pixel to surface. Finally, they perform estimation over the posterior with the Expectation-Maximization algorithm. The camera is tracked in the M-Step with regards to the background TSDF (due to foreground masks being inaccurate), after which the association probabilities are recomputed and object TSDF locations also tracked. The map is updated in the M-Step by integrating the new depth image into the SDF recursively with measured depth difference, latent variable prior and weights. Most importantly, the authors compare their method with MaskFusion \cite{maskfusion}, MID-Fusion \cite{xu2019mid} and Co-Fusion. Their approach outperforms Co-Fusion and MaskFusion when evaluated on the RGB-D dataset. They attribute their performance to tracking using direct SDF alignment in comparison to MaskFusion's ICP tracking with the static background. The authors highlight that \textcolor{red}{instead of masking out non-rigid dynamic objects such as human beings like their counterparts, they associate non-rigid objects to the object volumes rather than the background, enabling them to track the camera with respect to the background.}
\subsubsection{Surfels}

\subsubsection{Scene Graphs}
Rosinol et. al. \cite{rosinol20203d} introduced dynamic scene graphs. A node in a graph is modelled after a "spatial concept" and the edges as spatio-temporal relationships between them. The map is built on the basis of 5 layers of abstraction, which affords disambiguations between classes that could belong to foreground or background, be static or dynamic and be traversable or non-traversable. The last two layers of abstraction help group these entities according to their spatial relationships. Edges can represent relationships between spatial entities that aren't otherwise captured - like contact, co-visibility, distance and relative size. A semantic-mesh is constructed using Kimera \cite{rosinol2019kimera}, robot pose is tracked with IMU-aware optical flow and all objects other than humans are extracted with their CAD model or with unknown shape. Human beings are extracted from a panoptic 2D image using a Graph-CNN \cite{zhao2019semantic} and tracked. Tracking is contingent on the bounding box encapsulating the human having a minimum number of pixels and the feasible motion of joints in the meshes from one time step to the next. To exclude the human from the static mesh, they feed the "human-being mesh" back into the static mesh by using the free-space information available from ray-casting towards the depth of the human pixels. \textcolor{purple}{It is \textbf{unclear} how they will track dynamic objects other than human beings but the concept of \textbf{dynamic masking} may be generalizable to other applications such as oct-trees as well.} Finally, for topological parsing of the map, the authors convert the mesh to a 3D ESDF using VoxBlox \cite{oleynikova2017voxblox} and develop the hierarchical relationships previously described.


% \begin{table*}[t]
%     \centering
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{|c|cccccccccccc|}
%     \toprule
%       Work  & Mapping-Only & Geometric & Learning-Based & Semantic & LiDAR & Camera & discard fg & Scene Propagation & Map Repr. (post-processing) & Scene Flow & Code & Real-Time \\ \midrule
%       Cheng et. al \cite{cheng2020robust} & $\checkmark$ & OptFlow, depth  & CRF-RNN & $\checkmark$ & $\times$ & $\checkmark$ & $\checkmark$ & $\times$ & point cloud map & $\times$ & $\times$ & $\times$ \\
%       Brasch et al \cite{brasch2018semantic} & $\times$ & ORB, depth & $\checkmark$ & $\checkmark$ & $\times$ & monocular & $\checkmark$  & $\checkmark$ & $\times$ & $\times$ & $\times$ & $\checkmark$ \\
%       DynaSLAM \cite{dynaslam} & $\times$ & ORB, depth & Mask R-CNN & $\checkmark$ & $\times$ & RGB-D & $\checkmark$ & $\times$ & inpaint, feature mp & $\times$ & \href{https://github.com/BertaBescos/DynaSLAM}{$\checkmark$} & $\times$\\
%       DS-SLAM \cite{yu2018ds}& $\times$ & OptFlow, RANSAC & SegNet & $\checkmark$ & $\times$ & RGB-D & $\checkmark$ & $\times$ & semantic oct-tree & $\times$ & \href{https://github.com/ivipsourcecode/DS-SLAM}{$\checkmark$}&< 2Hz det. bn. \\
%       SOF-SLAM \cite{cui2019sof}& $\times$ & OptFlow, epigeom & SegNet & $\checkmark$ & $\times$ & RGB-D & $\checkmark$ & $\times$ & $\times$ & feature mp & $\times$ & $\checkmark$ Qual \\
%       DSO-Dynamic \cite{ma2019dsod} & pose & depth prediction & Mask R-CNN & to filter dynamic & $\times$ & RGB & $\checkmark$ & $\times$ & $\times$ & $\times$ & $\times$ & 8 fps \\
       
%       Chen et al. (Suma++) \cite{chen2019suma++} &  $\checkmark$ & ICP, vertex/normal map & RangeNet++ & $\checkmark$ & $\checkmark$ & $\times$ & $\checkmark$ & $\checkmark$-transforms & surfel (flood-fill) & $\times$ & \href{https://github.com/PRBonn/semantic_suma/}{$\checkmark$} & <2 Hz\\
%       SLAM++ \cite{salas2013slam++} & $\times$ & ICP-tracking, \cite{drost2010model} & $\times$ & obj DB & $\times$ & $\checkmark$ & $\checkmark$ ICP-gating fail & $\checkmark$ - transform & object (PPF), graph & $\times$ & \href{https://sourceforge.net/p/slam-plus-plus/wiki/Home/}{$\checkmark$} & 20 fps\\
%       Alcantarilla et. al. \cite{alcantarilla2012combining} & $\times$ & SF. motion l.h  & $\times$& $\times$ & $\times$ & $\checkmark$ & VO inliers w. motion l.h. & transform hist. & feature, 3D loc. tracks & $\checkmark$ & $\times$ & $\checkmark$ Qual\\
%       DOS-SLAM \cite{xu2019slam} & $\times$ & ORB, epigeom, SF. motion l.h. & YOLACT & $\checkmark$ & $\times$ & $\checkmark$ & $\checkmark$ & $\times$ cons. frames & semantic oct-tree & $\checkmark$ & $\times$ & 30 fps  \\
       
%       Zhong et. al. \cite{detect} & $\times$ & ORB k.p-3Dp match, motion prob. & SLAM-enhanced SSD& $\checkmark$  & $\times$ & RGB-D & for pose est. & k.f.$\xrightarrow[\text{no bg}]{\text{updates}}$ obj m.p.& object - dense PC w. id& $\times$ &$\times$& 2 fps det.\\
%       Schorghuber et al. \cite{schorghuber2019slamantic} & $\times$ & ORB, label consistency & \cite{yu2018deep}, 19 cl, 9fps & $\checkmark$ & $\times$ & stereo/mono & validate sd, init s, final sd  & \# obs. of m.p.  & 3D point (unclear) & $\times$ & \href{https://github.com/mthz/slamantic}{$\checkmark$} & $\times$ ?\\
%       Recurrent OctoMap \cite{sun2018recurrent} & $\checkmark$ \\
%       Fusion++ \cite{mccormac2018fusion++}&  $\times$ & ICP f2m track\cite{newcombe2011kinectfusion}, RANSAC & Mask R-CNN & $\checkmark$ & $\times$ & RGB-D & no dynamic track & TSDF: pose = $T_{ow}$, relocalize &  voxel, exist. prob.; object & $\times$ & \href{https://github.com/awaescher/Fusion}{$\checkmark$}& $\times$ - 4 Hz w/o g.o \\
%       MaskFusion \cite{maskfusion} & $\times$ &edginess, track: min(geom + photo) & Mask R-CNN & $\checkmark$ & $\times$ & RGB-D & $s_{tm}$ static indicator & $R_{tm}$, t=time, m=model & surfel (mask/geom->model) &  $\times$ & \href{https://github.com/martinruenz/maskfusion}{$\checkmark$}& >30 Hz gpu det.\\
%       Huang et. al \cite{huang2019clusterslam} & $\times$ & hier. clustering & $\times$ & $\times$ & $\times$  & stereo & $\times$ & cluster init. + tracked & cluster contains lms, traj & $\times$ & $\times$ & 7.1 Hz \\
       
%       DynSLAM \cite{barsan2018robust} & $\times$ & reconstruct: infiniTAM \cite{prisacariu2017infinitam} & depth-fusion: Disp-Net, ELAS & $\times$ & $\times$ & stereo & $\times$ & $\checkmark$ w/ a limit & voxel (artifact: garbage collection) & dynamic obj motion &  \href{https://github.com/AndreiBarsan/DynSLAM}{$\checkmark$} & $\checkmark$ - 2.5 Hz (seg bn) \\
%       Ushani et. al \cite{aushani-2018a} & N/A  & feature learning & loss fn., EM Algo. & $\times$ dyn. cl. compared & $\checkmark$ & $\times$ & fg/bg class. loss & $\times$ & occupancy grid & for dynamic objects &  \href{https://github.com/aushani/flsf}{$\checkmark$}& $\times$ \\ 
%       Dewan et. al \cite{dewan2016rigid} & N/A & SHOT \cite{tombari2010unique}, n-hood: mesh \cite{marton2009fast} & $\times$ & $\times$ & $\checkmark$ & $\times$ & N/A & N/A & trans. + rot. PC-PC & rigid scene flow & $\times$ & unknown \\
%       Wang et. al. \cite{wang2020coarse} \\
%       Jiang et. al. \cite{jiang2020local} \\
%       Rosinol et. al. \cite{rosinol20203d} & $\times$ & Odom: OptFlow, RANSAC \cite{rosinol2019kimera} & Track: \cite{zhao2019semantic}, Mesh: \cite{rosinol2019kimera} & $\checkmark$ & $\times$ & $\checkmark$ & Map: $\checkmark$, Track: $\times$ & $\checkmark$ & scene graph & $\times$ & $\times$ & $\times$ \\
%       Muglikar et. al. \cite{muglikar2020voxel} \\
%       Kochanov et. al. \cite{kochanov2016scene} & $\times$ &  & \cite{ovsep2016multi} (detect. by track) & semantics - $\checkmark$ & stereo & voxel grid \\
%       Vespa et. al. \cite{vespa2018efficient} & $\times$ & Odom: ICP, \cite{laine2010efficient} & $\times$ & $\times$ & $\times$ & $\checkmark$ & no dynamic, f2map & $\times$ & TSDF/Occ.Grid & $\times$ & $\times$ & $\checkmark  $ (10-40 Hz)\\
%       Xu et. al. \cite{xu2019mid} & $\times$ & odom + track: (ICP-geom + photo) & Mask-RCNN & $\checkmark$ & $\times$ & RGB-D & track: ICP & $\checkmark$ & TSDF + fusion : \cite{vespa2018efficient} & $\times$ & $\checkmark$ &  $\times$ (400 ms)\\
%       Streck et. al. \cite{strecke2019fusion} & $\times$ & \cite{bylow2013real} & Mask-RCNN & $\checkmark$ & $\times$ & $\checkmark$ & exc. cam. track. $\times$ & $\checkmark$ & TSDF/voxel & $\times$ & $\times$ & $\times$ ~2Hz\\
%       Henein et. al. \cite{henein2020dynamicslam}\\
%       Narita et. al. \cite{}\\
%       DynamicFusion \\
%       Co-Fusion \\
       
%       Wang et. al. \cite{wang2019real} \\
            
%         \bottomrule
%     \end{tabular}
%     }
   
%     \caption{Caption \mgj{Started looking good! this is going to be super useful.}}
%     \label{tab:my_label}
% \end{table*}


==> results_revised.tex <==


In this section, we firstly, describe our experimental setup and the datasets used to evaluate our framework against baselines. Then, we demonstrate the performance of the mapping system with qualitative results on synthetic and real datasets. Finally, quantitative results on single- and multi-view datasets using the proposed evaluation metric in Section \ref{sec:eval} are presented.

\subsection{Experimental Setup}
We first describe our (i) kernel design choices, (ii) then elaborate on the datasets used and (iii) lastly, discuss the scene flow networks used to obtain point cloud data.

\subsubsection{Kernel Design Choices}\label{sec:experiments}
In the mapping framework, every query voxel has 6 neighbours (one on each face). Weights from only the training points observed in each of the six neighbouring voxels are used in the calculation of both \eqref{eq:velocity} and \eqref{eq:velfree}.

We choose a sparse kernel~\cite{melkumyan2009sparse} as $\mathcal{K}_v^{\text{free}} = $
\begin{align}
\small 
    % \nonumber &\mathcal{K}_v^{\text{free}}(x,x') = \\
    \nonumber &\begin{cases}
        \sigma_1[(\frac{1}{3}(2 + \cos({\frac{2\pi d}{l_1}})(1 - \frac{d}{l_1}) + \frac{1}{2\pi}\sin({\frac{2\pi d}{l_1}})] & \text{if } d < l\\
        0 & \text{otherwise}
    \end{cases}
\end{align}
where \mbox{$d = \lVert x-x'\rVert$, $l_1 > 0$} the length scale and $\sigma_1$ the kernel scale parameter. To compute $\mathcal{K}_v$ in \eqref{eq:velocity}, we use an isotropic Mat\'ern kernel~\cite{stein1999interpolation}, \mbox{$\mathcal{K}_v(x,x') = \sigma_2[(1 + \frac{\pi d}{2l_2}) e^{-\frac{\pi d}{2l_2}}]$}, where $d = \lVert x-x'\rVert$, $l_2 > 0$ the length scale and $\sigma_2$ the kernel scale parameter.

Typically, the kernel length scales for both $\mathcal{K}_v$ and $\mathcal{K}_v^{\text{free}}$ are chosen with respect to the resolution of the map being built as it controls how much influence a point in a neighbouring cell has. In our experiments, $l_1$ is always twice the map resolution and $\sigma_1$ can be set once in the beginning according to the size of the point set and free-space sampling resolution.

\subsection{Data sets and Benchmarks:}

\noindent \textbf{Gazebo Simulation Environment:} To create an indoor synthetic data set, a Gazebo simulation environment was set up with multiple Turtlebots exploring a house. We mounted one robot (the ego-robot) with an omni-directional block laser scanner for data collection in the form of point clouds with \emph{positional information only}. To simulate dynamic objects in the environment, we have three other Turtlebots exploring the same house. Using a reactive planner, the robots avoid each other and obstacles in the environment. The collected data is processed using the Point Cloud Library (PCL) and annotated based on height into three labels - floor, robot and miscellaneous objects such as walls or cabinets. The scene flow for each scan is computed with FlowNet3D.\par 
\noindent \textbf{SemanticKITTI Data Set:} The SemanticKITTI data set~\cite{behley2019semantickitti} is a large-scale real driving data set based on the KITTI Vision Benchmark where semantic annotations and camera poses are provided for all sequences. Camera poses are estimated with SuMa \cite{behley2018efficient}, and semantic annotations are generated with RangeNet++\cite{milioto2019rangenet++}. Additional labels are provided to distinguish static objects from dynamic objects, such as person and moving-person. There are 22 sequences, out of which 11 sequences are provided with ground truth labels for training (00-07), validation (08) and testing (09-10). Sequence 11-21 do not come with ground truth semantic labels, but can be evaluated in a public leaderboard over the mean intersection-over-union (mIoU) metric. Since the most reliable ground truth model in a single-view dataset such as this one is the semantically-labelled point cloud, we use the same/generate a completed scene.
\noindent \textbf{CARLA Data Set:} \todo{write more} To generate a reliable ground truth model of the scene for evaluation of the global map, we obtain multiple views of the same scene and fuse the data into a voxel map. The voxel centers in the voxel map act as query points in the completeness experiments.

\subsubsection{Velocity Estimation}

For the SemanticKITTI and Gazebo simulation environment data set, we generate per-point velocities $\mathcal{V}_t$ with dense scene flow.
We chose a state-of-the-art deep learning architectures based on PointNet++\cite{PointNetPP} -  FlowNet3D \cite{flownet3d} : supervised method based on PointNet++ \cite{qi2017pointnet} which estimates scene flow between two successive point clouds $\mathcal{X}_{t-1}.$ %and $\mathcal{X}_t$%; 2) TLFPAD \cite{tlfpad} : self-supervised method based on PointNet++ \cite{PointNetPP} which incorporates temporal information from four point clouds $\mathcal{X}_{t-3:t}$. Predicted scene flow $\mathcal{V}_t$ is compared with the next point cloud $\mathcal{X}_{t+1} = \mathcal{V}_t + \mathcal{X}_t$.

Typically, implementations for scene flow estimation train on the XYZRGB fields, i.e., the point cloud includes both the position and colour information. We trained an adapted version of FlowNet3d on the KITTI 2015 Scene Flow data set \cite{menze2015object} and the FlyingThings driving data set \cite{mayer2016large} by only including position information for training. After obtaining the $\mathcal{V}_t$ from the networks, we perform egomotion-compensation on the point cloud by subtracting the mean flow of static classes.

As we only need velocity for moving objects, our mapping method can be applied when any kind of corresponding velocity information for $\{x_t^m \in \mathcal{X}_t \forall m \mathcal{M}\}$ is available. To demonstrate the performance of the mapping framework in the presence of true velocity, we obtain the ground truth velocity of dynamic objects from the CARLA simulator.

\subsection{Qualitative Results}

\subsection{Quantitative Results}


==> revision.tex <==
\newpage

%%% Revision changelogs:
%1. Remove parameter table and include it in supplementary?
%2. fastest way to get Scene flow? 
%TODO: Motivate this section from the introduction???
\section{Quantitative Evaluation on Dynamic Mapping Sub-tasks}

\subsection{Semantic Scene Reconstruction}

Let the ground truth model of the environment be denoted as $\mathcal{G}$ and our model (voxel map) as $\mathcal{M}.$ Let the rays from our current scan fall into a set of voxels denoted by $\mathcal{M}_v$. The voxels that are not seen in the current scan would then be $\mathcal{M}_o = \mathcal{M} - \mathcal{M}_v$. To compare the scene reconstruction between our model $\mathcal{M}$ and the ground truth $\mathcal{G}$, we employ two different map query methods introduced in \cite{seitz}: accuracy and completeness.

%create a diagram that shows G v/s M and how hole-filled M’ is made. (Basically, align them both together).

\subsubsection{Accuracy}
To evaluate the dynamic map created from the current scan, we pick a voxel $m \in \mathcal{M}_v$ and find its nearest neighbor $g_m \in \mathcal{G}$. The voxel $m$ is then evaluated against its nearest neighbor $g_m$. If we are comparing the accuracies of two mapping methods with different map representations, the query points $m \in \mathcal{M}_v$ could be different. Therefore, accuracy is a more representative metric for comparison when map representations are the same across two methods (in terms of resolution, map origin, etc). Therefore, we compare static-BKI (S-BKI) and dynamic-BKI (D-BKI) and compute the precision, recall and Jaccard scores across all classes.

%In practice, both $\mathcal{G}$ and $\mathcal{M}_v$ must have the same resolution and origin so $g_m$ and $m$ have the same voxel center $\in \mathbb{R}^3$.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\textwidth]{media/completeness.jpg}
    \caption{An illustration of the ground truth model as viewed from the robot's perspective. Rays pass through the voxels that are \textbf{observed} by the robot. For voxels that are unseen by the robot in the current scan, they could have been previously observed but are currently \textbf{occluded.} Alternatively, there could also be voxels that are \textbf{unexplored} by the robot but present in the ground-truth model created by the multi-view dataset.}
    \label{fig:gtmap}
\end{figure}

\begin{figure*}
    \centering
    \includegraphics{}
    \caption{Insert a graph with accuracy and completeness info? }
    \label{fig:my_label}
\end{figure*}

\subsubsection{Completeness}
To evaluate the completeness of the map, we estimate how much of the ground truth model is reconstructed correctly by $\mathcal{M}$. With completeness, we can compare the map inference performance across baselines with different map representations. When the ground truth model $\mathcal{G}$ is generated with multiple views, we can also assess map inference in the presence of occlusions (with $\mathcal{M}_o$). 

We pick a voxel $g \in \mathcal{G}$ and find its nearest neighbor in $m_g \in \mathcal{M}$. If the distance between $g$ and $m$ is greater than a certain margin, we consider that $g$ is currently unexplored by the robot (and not covered by $\mathcal{M}$) and do not include these pairs in the evaluation. These voxels are shown in the rightmost column in Fig. ~\ref{fig:gtmap}.

To keep the evaluation relevant to dynamic mapping, we adopt different approaches according to whether $g$ is static or dynamic:
\begin{enumerate}

\item If $g$ is static: In this case, for any $g \in \mathcal{G}$, we evaluate semantic accuracy for nearest neighbors $m_g \in \mathcal{M}_v$ and $m_g \in \mathcal{M}_o.$ These are the visible and occluded voxels shown in Fig.~\ref{fig:gtmap}.

\item If $g$ is dynamic: As only dynamic objects in $\mathcal{M}_v$ are seen by the robot, we evaluate on semantic accuracy for all $m_g \in \mathcal{M}_v$. We do not evaluate on $\mathcal{M}_o$ as these voxels in the map are occluded and could have a different state from the last time it was observed by the robot. These voxels are shown with the legend "visible" in Fig.~\ref{fig:gtmap}.

\end{enumerate}

For this task, we pick two data sets:
\subsubsection{Single-View Dataset (SemanticKITTI)}
We picked 4 sequences from the SemanticKITTI dataset that are representative of the challenges faced while driving in dynamic environments - highways (sequence 01) on faster speeds, countrysides (sequence 03) and cities (sequence 06) on medium speed, and residential areas in cities (sequence 10) on slow speed. 
\begin{table*}[ht]
% \footnotesize
\centering
\caption{Mean IoU on SemanticKITTI data set sequences 01, 03, 06 \& 10 ~\cite{behley2019semantickitti} for 26 semantic classes.}
\label{table:semantickitti}
\resizebox{\textwidth}{!}{
\begin{tabular}{llllcccccccccccccccccccccccc}
% \toprule
% \multicolumn{3}{c|}{Method}
{\bf Method} & 

\cellcolor{scarColor}\rotatebox{90}{\color{white}Car} &
\cellcolor{sbicycleColor}\rotatebox{90}{\color{white}Bicycle} &
\cellcolor{smotorcycleColor}\rotatebox{90}{\color{white}Motorcycle} &
\cellcolor{struckColor}\rotatebox{90}{\color{white}Truck} & 
\cellcolor{sothervehicleColor}\rotatebox{90}{\color{white}Other Vehicle} & 
\cellcolor{spersonColor}\rotatebox{90}{\color{white}Person} &
\cellcolor{sbicyclistColor}\rotatebox{90}{\color{white}Bicyclist} &
\cellcolor{smotorcyclistColor}\rotatebox{90}{\color{white}Motorcyclist} &
\cellcolor{sroadColor}\rotatebox{90}{\color{white}Road} &
\cellcolor{sparkingColor}\rotatebox{90}{\color{white}Parking} &
\cellcolor{ssidewalkColor}\rotatebox{90}{\color{white}Sidewalk} &
\cellcolor{sothergroundColor}\rotatebox{90}{\color{white}Other Ground} &
\cellcolor{sbuildingColor}\rotatebox{90}{\color{white}Building} &
\cellcolor{sfenceColor}\rotatebox{90}{\color{white}Fence} &
\cellcolor{svegetationColor}\rotatebox{90}{\color{white}Vegetation} &
\cellcolor{strunkColor}\rotatebox{90}{\color{white}Trunk} &
\cellcolor{sterrainColor}\rotatebox{90}{\color{white}Terrain} &
\cellcolor{spoleColor}\rotatebox{90}{\color{white}Pole} &
\cellcolor{strafficsignColor}\rotatebox{90}{\color{white}Traffic Sign} &
\cellcolor{scarColor}\rotatebox{90}{\color{white} Car-Moving} &
\cellcolor{sbicyclistColor}\rotatebox{90}{\color{white} Bicyclist-Moving} &
\cellcolor{spersonColor}\rotatebox{90}{\color{white} Person-Moving} &
\cellcolor{smotorcyclistColor}\rotatebox{90}{\color{white} Motorcylist-Moving} &

\cellcolor{sothervehicleColor}\rotatebox{90}{\color{white} Other Vehicle-Moving} &
\cellcolor{struckColor}\rotatebox{90}{\color{white} Truck-Moving} &

\rotatebox{90}{\bf Average}\\ \hline 

\vspace{-2mm} \\
S-BKI & 0.946 & 0.593 & 0.411 & 0.495 & 0.461 & 0.273 & 0.0 & 0.0 & 0.907 & 0.663 & 0.748 & 0.26 & 0.906 & 0.656 & 0.857 & 0.727 & 0.711 & 0.637 & 0.694 & 0.756 & 0.64 & 0.656 & 0.329 & 0.221 & 0.012 & 0.542 \\
 D-BKI & 0.946 & 0.676 & 0.638 & 0.413 & 0.388 & 0.125 & 0.017 & 0.002 & 0.907 & 0.65 & 0.745 & 0.323 & 0.926 & 0.66 & 0.858 & 0.72 & 0.689 & 0.631 & 0.614 & 0.749 & 0.683 & 0.657 & 0.119 & 0.001 & 0.0 & 0.525 \\
Kochanov et. al. & 0.946 & 0.593 & 0.411 & 0.495 & 0.461 & 0.273 & 0.0 & 0.0 & 0.907 & 0.663 & 0.748 & 0.26 & 0.906 & 0.656 & 0.857 & 0.727 & 0.711 & 0.637 & 0.694 & 0.756 & 0.64 & 0.656 & 0.329 & 0.221 & 0.012 & 0.542 \\
\bottomrule
\end{tabular}
}
% \squeezeup
\label{tab:single_view_comp}
\end{table*}
\subsubsection{Multi-view Dataset (CARLA)}

For the CARLA dataset, we split the dataset into 5 scenarios comprising of 200 scans each and evaluate how the map fares in each.

\begin{table}[t]
% \footnotesize
\centering
\caption{Accuracy on the CARLA dataset}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{llllcccccccccccccccccccccccc}
% \toprule
% \multicolumn{3}{c|}{Method}
{\bf Indicator} & 
\multicolumn{1}{l}{\bf Method}&
\cellcolor{smotorcyclistColor}\rotatebox{90}{\color{white}Free Space} &
\cellcolor{struckColor}\rotatebox{90}{\color{white}Vehicle} &
\cellcolor{spersonColor}\rotatebox{90}{\color{white}Pedestrian} &
\cellcolor{sroadColor}\rotatebox{90}{\color{white}Road} &
\cellcolor{sbuildingColor}\rotatebox{90}{\color{white}Building} & 
\cellcolor{sothervehicleColor}\rotatebox{90}{\color{white}Sidewalk} & 

\cellcolor{scarColor}\rotatebox{90}{\color{white}Traffic Sign} &
\rotatebox{90}{\bf Average}\\ \hline 

\vspace{-2mm} \\
\multirow{2}{*}{Precision}
& S-BKI &  & & & & &  \\
& D-BKI (Ours) & & & & & & \\
\bottomrule
\vspace{-2mm} \\
\multirow{2}{*}{Recall}
& S-BKI &  & & & & &  \\
& D-BKI (Ours) & & & & & & \\
\bottomrule
% \vspace{-2mm} \\
% \multirow{2}{*}{Jaccard Score}
% & S-BKI &  & & & & &  \\
% & D-BKI (Ours) & & & & & & \\
% \bottomrule
\end{tabular}
}
% \squeezeup
\label{tab:carla_acc}
\end{table}

\begin{table}[t]
% \footnotesize
\centering
\caption{Completeness on the CARLA dataset}
\label{table:completeness}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{llllcccccccccccccccccccccccc}
% \toprule
% \multicolumn{3}{c|}{Method}
{\bf Indicator} & 
\multicolumn{1}{l}{\bf Method}&
\cellcolor{smotorcyclistColor}\rotatebox{90}{\color{white}Free Space} &
\cellcolor{struckColor}\rotatebox{90}{\color{white}Vehicle} &
\cellcolor{spersonColor}\rotatebox{90}{\color{white}Pedestrian} &
\cellcolor{sroadColor}\rotatebox{90}{\color{white}Road} &
\cellcolor{sbuildingColor}\rotatebox{90}{\color{white}Building} & 
\cellcolor{sothervehicleColor}\rotatebox{90}{\color{white}Sidewalk} & 
\cellcolor{scarColor}\rotatebox{90}{\color{white}Traffic Sign} &
\rotatebox{90}{\bf Average}\\ \hline 

\vspace{-2mm} \\
\multirow{2}{*}{Precision}
& S-BKI &  & & & & &  \\
& D-BKI (Ours) & & & & & & \\
& Kochanov et. al. & & & & & \\
\bottomrule
\vspace{-2mm} \\
\multirow{2}{*}{Recall}
& S-BKI &  & & & & &  \\
& D-BKI (Ours) & & & & & & \\
& Kochanov et. al. & & & & & \\
\bottomrule
% \vspace{-2mm} \\
% \multirow{2}{*}{Jaccard Score}
% & S-BKI &  & & & & &  \\
% & D-BKI (Ours) & & & & & & \\
% \bottomrule
\end{tabular}
}
% \squeezeup
\label{tab:carla_comp}
\end{table}

\subsection{Semantic Segmentation}

\newpage
